How Does Conversation Length Impact User's Satisfaction? A Case Study of Length-Controlled Conversations with LLM-Powered Chatbots

Users can discuss a wide range of topics with large language models (LLMs), but they do not always prefer solving problems or getting information through lengthy conversations. This raises an intriguing HCI question: How does instructing LLMs to engage in longer or shorter conversations affect conversation quality? In this paper, we developed two Slack chatbots using GPT-4 with the ability to vary conversation lengths and conducted a user study. Participants asked the chatbots both highly and less conversable questions, engaging in dialogues with 0, 3, 5, and 7 conversational turns. We found that the conversation quality does not differ drastically across different conditions, while participants had mixed reactions. Our study demonstrates LLMs' ability to change conversation length and the potential benefits for users resulting from such changes, but we caution that changes in text form may not necessarily imply changes in quality or content.

==> Sections/2-related-work.tex <==
\kenneth{TODO Steven and Alan: Move citations to the newly written Related Work section.}

In the field of conversational assistants, much research has been devoted to understanding the broader context in which users interact with these systems, including their use in everyday household scenarios~\cite{porcheron2018voice, sciuto2018hey}. 
% and what people value in conversation and \cite{clark2019makes}. 
Within Ubiquitous Computing, a significant body of work has been done on ``context-aware computing''~\cite{dey2018context}. 
This research often revolves around enhancing conversational assistants with the ability to sense user context~\cite{acer2022city, chan2020prompto}. For example, using ambient acoustic data to detect human activities like typing or walking~\cite{park2020augmenting} and utilizing respiration sensor to assist users in managing breathing patterns~\cite{shamekhi2018breathe}.\kenneth{If possible, add one more example.} 
Likewise, in Affective Computing, efforts have been made to adjust conversational strategies based on detected user emotions-- in which the ``context'' is the emotion-- whose goals were often to resonate with users' emotions and thus enhance user engagement~\cite{ghandeharioun2019emma, casas2021enhancing, samrose2020mitigating, yang2019understanding}.
However, despite the intriguing research that took user context into account, the majority of dialogue systems research, including recent LLM-based chatbots, remained largely disconnected from such considerations~\cite{ham-etal-2020-end, OpenAI2023GPT4TR,OpenAI}.\steven{should we put some dialogue system research and gpt papers here} \alan{yeah but probably just 1-2 that's representative, `just to make a point' sort of deal}\steven{sure}
In contrast, the natural language processing (NLP) and dialogue system communities focus primarily on producing accurate responses without considering the user's specific situation; most benchmark datasets for dialogue systems lack user context information~\cite{zhou-etal-2022-towards-identifying,dziri-etal-2022-evaluating, lowe-etal-2015-ubuntu}.\kenneth{Add a few datasets that do not have user context.}
The phrase ``context-aware'' conversational systems in NLP literature often refers to those that consider the domain or user's chat history, emphasizing the content of the conversation over the user's situation~\cite{duvsek2016context,zhou-etal-2016-context,10.1145/3474085.3475234,snell-etal-2022-context}.\kenneth{Add context aware dialogue system from NLP conferences.}
Consequently, the systems considering user context have typically been developed only as ad-hoc projects with specific sensing capabilities, such as emotion-detection or environmental-sensing features~\cite{Majumder_Poria_Hazarika_Mihalcea_Gelbukh_Cambria_2019,lee-etal-2019-convlab}.

In this paper, we respond to this gap by advocating \textbf{a separation of conversation format from content, with situational information mainly influencing format}. 
This separation offers two-fold advantages:
First, it ensures that effective existing dialogue systems like ChatGPT maintain their focus on content. 
This way, they can continue enhancing their capabilities using current datasets, model frameworks, and infrastructure while potentially benefiting from additional situation awareness. 
Second, it provides a straightforward path for researchers focused on user context to leverage the advancements of LLM-powered chatbots in their studies. 
With the impressive capabilities of modern LLMs, tailoring a response to suit a user's situation is now more attainable than ever.

To emphasize our unique approach, we have chosen to use ``situation'' instead of more commonly used terms like ``context'' or ``scenarios.''


% ~\cite{goar2023conversational} 
% Users input their queries or statements in written form, and ChatGPT generates human-like responses in real-time, also in text format.
% This text-based modality allows for natural language conversations with the AI model, enabling users to ask questions, make statements, and receive contextually relevant responses.

% ~\cite{sakirin2023user}
% 70\% of users preferred ChatGPT-powered conversational interfaces over traditional techniques, citing convenience, efficiency, and personalization, where traditional techniques refer to conventional techniques or approaches that have been used before the introduction of ChatGPT-powered conversational interfaces.
% 85\% of participant who used ChatGPT-powered conversational interfaces reported high levels of satisfaction. 
% \steven{goar2023conversational and sakirin2023user didn't explicitly mentioned the modality of interaction with ChatGPT, but it can be inferred that the default modality of interaction with ChatGPT is through text-based conversations. }
% ~\cite{wang2023zero} The study used ChatGPT to in cross-lingual summarization task, which was done by text prompts
%\bigskip


% \paragraph{Context-aware computing}
% % In dialog system research, context usually means the conversation itself rather than the environments or scenarios \avon{cite some papers}. Research in dialog system community \avon{or NLP community?} mainly focuses on studying users' perceptions and behaviors in terms of the change of the conversation content, such as using chat history for personalization. 
% %
% Research in ubiquitous computing has long studied context-aware computing~\cite{dey2018context}. In ubiquitous computing, contexts have broader meanings, including environments or scenarios. Some of them studied context-aware conversational systems, yet the studies mainly focus on creating context-aware sensing techniques~\cite{acer2022city, park2020augmenting, chan2020prompto}\avon{cite more?}. For example, \citet{park2020augmenting} studied how ambient acoustic data can be used to detect human motions, like typing/clicking, television, and walking, and enable conversational agents to provide context-aware outputs.
% %
% Our research is situated at the intersection of the two research communities. We understand how to design conversational agents in terms of various environments or situations by studying users' behaviors and perceptions towards conversational agents' modalities and configurations in various situations.

% \paragraph{How do users alter their communication approach or preferences when their situation changes?}
% %The digital era has witnessed an ever-increasing shift towards voice-enabled conversational agents and interfaces. As they become more ingrained in our daily lives, it is crucial to understand the dynamics of user interactions and preferences in varying situations. 
% The digital era has witnessed an ever-increasing shift towards conversational agents and interfaces. As they become more ingrained in our daily lives, manifesting in mobile devices, smart speakers, and automotive systems, 
% %nonetheless, we do not know if users need different modalities in different situations.
% it is crucial to understand the dynamics of user interactions and preferences in varying situations.
% % 
% %\avon{Simplified version} Prior studies have investigated different input modalities of conversation agents, including voice-based, text-based, and multi-modal~\cite{ziman2018factors}\avon{more citations?}. Previous research has also examined the differing perceptions and reactions of various user groups when interacting with voice-based agents. These studies have investigated distinctions related to users' races~\cite{wenzel2023can}, ages~\cite{mehrotra2016embodied}, technical backgrounds~\cite{myers2019impact}, and various other factors~\cite{brewer2018accessible}. Researchers have designed multi-modal conversational agents that adapt to various kinds of users~\cite{aneja2021understanding}.
% Prior studies have investigated different modalities. In a study~\cite{ziman2018factors}, senior participants' perceptions of voice-based and text-based user interfaces were examined. Although a greater number of individuals found the voice-enabled interface to be user-friendly, they still favored the text input interface. This preference was attributed to several factors: users found the voice system to be engaging, but it required memorizing extensive commands before performing searches, and lacked features such as partial editing, auto-filling, and suggestions. 
% % \steven{need to find paper about mobile information seeking and multi modal information seeking}
% % Unlike the studies mentioned previously, which primarily investigate under single environments, our first research case delves deeper into the exploration of how users' preferences evolve across a range of diverse situations
% %
% %\textit{Different groups of users.} 
% In addition, previous research has examined the differing perceptions and reactions of various user groups when interacting with voice-based agents. These studies have investigated distinctions related to users' races~\cite{wenzel2023can}, ages~\cite{mehrotra2016embodied}, technical backgrounds~\cite{myers2019impact}, and various other factors~\cite{brewer2018accessible}\avon{if we say "various", should we have more citations here?}. Researchers have designed multi-modal conversational agents that adapt to various kinds of users~\cite{aneja2021understanding}.
% However, these lines of studies did not consider the modalities of conversational agents in terms of different situations.

% There are some studies that consider conversational input modalities in different situations.
% %\textit{Different types of scenarios.} 
% In a survey on conversational user interfaces~\cite{jaber2020conversational}, participants showed a preference for speech-based input when expressing their interpretations. However, in a usability test conducted on an in-car speech interface, users favored the barge-in feature, allowing them to regain control from the system, over using a voice-only system. Since these studies were carried out in diverse scenarios, our study aims to explore how users may adapt their preferences in response to changing situations.
% % 
% In our study, we used a conversational agent rather than a search engine, boasting capabilities akin to those of a highly sophisticated human agent. Furthermore, our primary scenario focuses on multi-tasking complex tasks. 

% ~\cite{begany2016factors}
% The user expressed discomfort when \textbf{speaking to the system}. User cannot edit or partially delete the quires in the spoken system.
% When users do not trust the spoken system or they have some concerns with using it, they tend to prefer the textual input system.
% Participants were impressed by the high accuracy of the voice recognition.
% A few participants emphasized the significance of editing or partially deleting queries within the spoken system.

% Suggested to have: 
%     1. quick editing and deleting
%     2. hybrid systems that combine both spoken system and textural input interface
%     3. spoken system used for simple task and textual input system for complex task

% ~\cite{wenzel2023can}
% Study aimed to understand if \textbf{speech recognition errors} in HCI may mirror the same effects as misunderstandings in cross-race community.
% Black participants were more negatively impacted by interacting with a more error-prone voice assistant compared to white participants
% Back participants in higher error condition exhibited higher levels of self-consciousness, lower levels of positive affect and self-esteem, and less favorable evaluations of the technology compared to black participants in low-error condition. White participants were largely unaffected by the error rate. 

% ~\cite{cho2019hey}
% The finding emphasize the important of considering both modality and user privacy concerns when designing \textbf{voice assistance}
% In conversation, when the information being asked was less sensitive in nature, voice interaction elevated the feeling of having a social conversation between user and the voice assistant
% There is no significant effects of device difference on user perception and attitude when sensitive level is higher.
% Text-only health information was easier to understand compared to voice message.


% ~\cite{reeves2018not}
% The \textbf{voice interface agent} like Alexa does not align with the reality of how these devices actually function. 
% Voice interfaces are designed for alone-at-a-time interactions, which hinders their ability to handle the complex and multi-activity nature of the real world
% HCI fields need to consider the practical and moral aspects of embedding voice interfaces into everyday life and whether they can truly be classified as conversations. 

% ~\cite{porcheron2018voice}
% Aim to understand the conversational methods employed by participants to accomplish tasks with the \textbf{voice device }and how its use is regulated within social dynamics of the home
% The device is not traded as a separate participant. It was integrated into ongoing activities
% The study emphasizes the importance of understanding how devices like the Echo are regulated within social settings and how they become part of ongoing cooperative activities

% ~\cite{mehrotra2016embodied}
% This paper describes the design and development of an \textbf{embodied conversational agent (ECA)} that provides a social interface for older adults.
% Senior people are not afraid of autonomous systems and their attitude improve after interacting with the system.
% Elder people preferred a friendly personality for the ECA, without the need for a life story or a strong character

% ~\cite{cha2021exploring}
% \textbf{Voice-enabled conversational agents} have the potential to assist adolescents diagnosed with autism spectrum disorder (ASD) in addressing their daily challenges.

% ~\cite{myers2019impact}
% Participants with more programming experience did not have wide-spread impact on performance metric and they were more curt with the \textbf{voice system}. Participants with increased VUI experience took
% less time with the tasks. Participant with more technical-background exhibit a trail-and-error approach to better understand the system and received a higher performance score. 


% ~\cite{dingler2021use}Conversational agents in digital health have the potential to make healthcare services and applications more widely accessible and personalized.

% ~\cite{brewer2018accessible}
% The paper emphasizes the importance of accessible voice interfaces for older adults and people with disabilities, as they lower the barriers of entry and use due to not requiring motor skills for text input through a keyboard.
% The workshop aims to explore recent advances in accessibility and voice interface research, situate voice-based accessibility in prior work and existing theoretical frameworks, discuss open challenges in the design of voice-based systems, and identify opportunities for interdisciplinary collaboration in this field

% ~\cite{seymour2021exploring}
% The paper explores the nature of relationships between users and voice assistants, such as Alexa and Google Assistant, and how these relationships correlate with trust and anthropomorphism
% It highlights the concerns raised over how the social nature of voice assistants might shape our interactions with them
% The paper aims to understand the similarities and differences between human relationships with voice assistants and relationships with other humans.
% The shift towards conversational interfaces and the social nature of voice assistants raise ethical concerns that designers need to consider when designing future products

% ~\cite{kuang2023collaboration}
% This paper explore the use of a conversational assistant for UX analysis, like what range of questions that UX evaluators are interested in asking, while we are interested in how users respond when communication method is changed in a conversational system.
% The \textbf{text assistant} was perceived as significantly more efficient.
% Participants using the text assistant asked more questions than those using the voice assistant.


% ~\cite{kang2017understanding}
% Speaking condition had a higher dropout rate than text input.

%\kenneth{TODO Steven: Add reference here.}

% \paragraph{How do users respond when a conversational system changes its communication method?}\steven{output modalities} 

% \steven{find paper that when changing output to users, how user will react. That is why we want to modify conversation length to see the user satisfaction}



% In a study that compared single-chatbot and multi-chatbot scenarios~\cite{chaves2018single}, researchers observed no notable differences in conversation structure between the two scenarios. Nevertheless, users expressed experiencing greater confusion during multi-chatbot interactions.
% The study found that proactive behaviors of conversational agents have the potential to disrupt sequential coherence while also aiding users in exploring a knowledge database~\cite{chaves2018single}. 
% Our study 2 is dedicated to understanding how our conversation agent can strategically adapt the length of a conversation to match specific situations, all with the goal of maximizing user benefits.

% Another study investigated the impact of incorporating conversational fillers into voice-based conversational agents on user perception~\cite{jeong2019exploring}. The insertion of these fillers was noted to result in a perception of reduced intelligence, with no statistically significant alteration in the perception of human-likeness. However, this modification appeared to enhance the entertainment value of social-oriented conversations.

% A previous study delved into the difficulties associated with emotional awareness and interactive realism in embodied conversational agents, achieved through aligning the conversational and expressive style of the user~\cite{aneja2021understanding}. The findings of the study demonstrated that the suggested agent had the capability to mirror the emotions of the participant, resulting in a notably more captivating conversational experience.

% Rather than relying on users' emotions, study 2 is centered on evaluating user satisfaction with their conversational experience when the chatbot extends the dialogue based on questions.

% In specific domains like health care, the majority output modality is text-only~\cite{tudor2020conversational}





% ~\cite{ziman2018factors}
% For searching task, though more people found that \textbf{Voice/Touch interface} is easy to use, they still prefer text input interface
% User need to memorize lots of things before using VTI 
% There is no suggestion for speaking like typing (auto fill, suggested questions)

% ~\cite{lister2020accessible}
% This paper reviews current guidance on accessible design for \textbf{conversational user interfaces (CUIs)} and highlights the potential benefits for people with disabilities.
% 1. Chatbox 
% 2. Interactive Voice Response (pre-recorded audio and specific response options)
% 3. Vistual assistant (Siri, Cortana)
% 4. Voice-activated personal assistant (VAPA). Alexa, Google assistant

% Conversational User Interface challenge includes 1) the person need to communicate additional or changing needs, request guidance, and avoid repetition of information, 2) CUI has to design to be fit for users who need more time to make responses. \steven{Based on the paper, CUI has to design to tailor user's background, like some users may need more time}

% ~\cite{jaber2020conversational}
% Combined speech-based text entry is 3x faster than keyboard
% Results showed that participants preferred to speak their
% interpretation of the CAPTCHA rather than typing it
% Even speech-based input works better when the number amount of text is small, there is no evident that CUI can replace the keyboard

% Regarding to usability test on an -in-car speech interface, user prefer the barge-in feature that wrestle back control from the system than using voice-alone system


% ~\cite{rzepka2022voice}
% Research on the preference between voice assistants and text assistants in customer service encounters is inconclusive, as it depends on the task and context of the interaction.
% Speaking is faster and easier, but listening to the voice assistant's answers reduces interaction speed, making text-based conversations relatively more efficient.
% Customers' enjoyment of text-based interaction increases for experiential tasks, while their enjoyment of speech-based interaction does not depend on the task. This could be due to the novelty effect of speech interaction.
% Contrary to the assumption, higher goal-directedness weakened the effect of speech on customers' cognitive effort, while text-based interaction resulted in lower cognitive effort for goal-directed tasks.
% The study shows that speech interactions have significant utilitarian and hedonic benefits compared to text interactions, positively impacting customers' service \textbf{satisfaction}.

% ~\cite{chaves2018single}
% The paper compared single and multi-chatbot scenarios and found no significant difference in conversation structure between the two scenarios. However, the users from the study reported more confusion in multi-chatbot interaction.

%\kenneth{TODO Steven: Add reference here.}

==> tables/slackbot-turk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\centering \small
\begin{tabular}{@{}lllccccc@{}}
\toprule
\textbf{} & \textbf{} & \textbf{} & \textbf{\slackBaseline} & \textbf{} & \multicolumn{3}{c}{\textbf{\slackBot}} \\ \cmidrule{4-4} \cmidrule{6-8}
\textbf{} & \textbf{} & \textbf{Converasbility} & \textbf{No Conversation} & \textbf{} & \textbf{N=3} & \textbf{N=5} & \textbf{N=7} \\ \midrule
\textbf{} & \multirow{2}{*}{\textbf{\# Dialogue}} & \textbf{High} & 44 &  & 9 & 11 & 12 \\
\textbf{} &  & \textbf{Low} & 28 &  & 15 & 10 & 12 \\ \midrule
\multirow{2}{*}{\textbf{Q$_1$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Helpfulness\\ (Strongly Disagree -\textgreater Strongly Agree)\end{tabular}}} & \textbf{High} & - &  & - & $\dagger$ & $\dagger$ \\
 &  & \textbf{Low} & $\bigstar$ &  & $\bigstar$ & - & - \\ \midrule
\multirow{2}{*}{\textbf{Q$_2$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Quantity\\ (Too Little -
\textgreater Too Much)\end{tabular}}} & \textbf{High} & $\diamondsuit$ &  & - & $\diamondsuit$ & - \\
 &  & \textbf{Low} & - &  & - & - & - \\ \midrule
\multirow{2}{*}{\textbf{Q$_3$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Relevance\\ (Strongly Disagree -\textgreater Strongly Agree)\end{tabular}}} & \textbf{High} & - &  & - & - & - \\
 &  & \textbf{Low} & - &  & - & - & - \\ \midrule
\multirow{2}{*}{\textbf{Q$_4$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Repetitiveness\\ (Strongly Disagree -\textgreater Strongly Agree)\end{tabular}}} & \textbf{High} & $\clubsuit$ &  & $\heartsuit$ & -& $\clubsuit$ $\heartsuit$ \\
 &  & \textbf{Low} & - &  & - & - & - \\ \midrule
\multirow{2}{*}{\textbf{Q$_5$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Clarity\\ (Strongly Disagree -\textgreater Strongly Agree)\end{tabular}}} & \textbf{High} & $\spadesuit$ &  & $\square$ & -& $\spadesuit$ $\square$ \\
 &  & \textbf{Low} & - &  & - & - & - \\ \midrule
 \multirow{2}{*}{\textbf{Q$_6$}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Ambiguity\\ (Strongly Disagree -\textgreater Strongly Agree)\end{tabular}}} & \textbf{High} & $\#$ &  & - & $\blacksquare$ & $\#$ $\blacksquare$ \\
 &  & \textbf{Low} & $\triangle$ &  & $\triangle$ & - & - \\ \bottomrule
\end{tabular}
\caption{Scores of the MTurk evaluation. Score pairs that passed the Chi-Squared Test are denoted by 
$\dagger$ (p-value = 0.046),
$\bigstar$ (p-value = 0.026),
$\diamondsuit$ (p-value = 0.041),
$\clubsuit$ (p-value = 0.013),
$\heartsuit$ (p-value = 0.01),
$\spadesuit$ (p-value = 0.022),
$\bigcirc$ (p-value = 0.015),
$\#$ (p-value = 0.009),
$\blacksquare$ (p-value = 0.032),
and $\triangle$ (p-value = 0.005). 
}
\label{tab:slackbot-turk}
\end{table*}
